Characterizing Branching Processes from Sampled Data

Branching processes model the evolution of populations of agents that randomly generate offsprings. These processes, more patently Galton-Watson processes, are widely used to model biological, social, cognitive, and technological phenomena, such as the diffusion of ideas, knowledge, chain letters, viruses, and the evolution of humans through their Y-chromosome DNA or mitochondrial RNA. A practical challenge of modeling real phenomena using a Galton-Watson process is the offspring distribution, which must be measured from the population. In most cases, however, directly measuring the offspring distribution is unrealistic due to lack of resources or the death of agents. So far, researchers have relied on informed guesses to guide their choice of offspring distribution. In this work we propose two methods to estimate the offspring distribution from real sampled data. Using a small sampled fraction of the agents and instrumented with the identity of the ancestors of the sampled agents, we show that accurate offspring distribution estimates can be obtained by sampling as little as 14% of the population.

==> discussion.tex <==
\section{Discussion}\label{sec:discussion}

%%other interpretation of the sampling model
%In Section~\ref{sec:model} we discussed two different sampling models: one that
%has a fixed number of targets and the other (used in this work) where
%each node is chosen as a target with probability $p$. Besides the fact that
%the latter model is mathematically more tractable than the former, it also has
%an alternative interpretation to that of modeling traceroutes from an origin node.
%We can think that no traceroute is performed but instead, nodes spontaneously advertise with
%probability $p$ all their ascendants. In fact, this is the scenario assumed in the study
%of petition letters in \cite{Chierichetti11}.

%%simple way to determine whether a tree is subtree of another
%Independently of the interpretation in use, the sampling model provides a
%unified
%and simple
%way to compute the probability of observing a sample $S$ given the tree $G$ (see
%eq.~\eqref{eq:probSgivenG}). The only caveat is that we need to determine whether $S$
%is a subtree of $G$. Although clever algorithms exist to verify this assertion,
%we propose a simple recursive way to do it. Let $G_1,\dots,G_{d_v}$ denote the
%subtrees connected to the root $v$ in $G$. Define $S_1,\dots,S_{d_u}$
%analogously w.r.t. the root $u$ in $T$. Clearly, if $d_u > d_v$, $S$ cannot be a
%subtree of $G$. Otherwise, find an injection  $f: S_i \rightarrow G_j,\,i=1,\dots,d_u$
%such that $S_i$ is a subtree of $G_j$ for all $i$.
%$T$ is a subtree of $G$ if and only if one such injection can be found.

%%why couldn't get MCMC to work with large tree
%Verifying if $S$ is a subtree of $G$ more efficiently would benefit both \Exact\
%and \Approx. However, using the na\"ive algorithm is not the reason why we
%couldn't use \Approx\ with the large size problems. In fact, it is due to a
%poor choice of $\btheta_0$ when picking a $g(G)$ to sample from. Since we use
%the uniform distribution, the probability that a node has $100$ children is the
%same as the probability that it has one single child. The average offpspring
%count in this case is $50.5$, which means that a proposal that adds a new branch
%to the root will augument the tree by $\approx 6.6$ million nodes on average.
%Hence this choice of $\btheta_0$ can rapidly consume all memory resources. Even if
%memory was infinite, this choice would generate trees very unlikely to have
%generated $S$: a very large branch was added to the tree, but none of its nodes
%were observed! This leads to vanishing acceptance ratio figures.
%As a
%guideline, we suggest $\btheta_0$ to be chosen so that the generated trees fit
%in the computer memory with high probability.

%%average issue
%In our description of \Level, we assumed that the average offspring $\bar{d}$ is known.
%However, when this is not the case, a fixed point mechanism can be used to
%iteratively estimate the offspring distribution and then the new average until
%it converges. Intuitively,
%an initial overestimate for $\bar{d}$ implies in overestimating the size of the
%subtrees connected to the nodes and consequently the probability of sampling
%edges. Therefore, \Level\ will underestimate the number of unobserved edges and
%yield an estimate of the offspring distribution biased towards a smaller average.
%The case of an intial underestimate for $\bar{d}$ is analogous. The initial
%guess could be the average degree of nodes from the first generations in the
%sample, whose edges have a relatively high probability of being sampled.

Recall from Section~XXX that $\btheta_0$ can be any distribution.
However, the more similar it is to $\btheta$, the better is the convergence of the MCMC.
When estimating the offspring distribution in medium size problems, we shall
assume that $\btheta_0$ is binomial and set its parameters so that the average
is $\bar{d}$. Note that this implies assuming that the average number of offsprings can be estimated.
In fact, we can obtain a down estimate for the
average by simply taking the average of the observed node degrees from the first generations in the
sample, whose edges have a relatively high probability of being sampled.

%But we could go even further and re-run the \Approx\
%using the previous estimate $\hat{\btheta}$ as the new $\btheta_0$.
%In regards to the previous assumption, we could obtain an estimate for the
%average by taking the average degree of nodes from the first generations in the
%sample, whose edges have a relatively high probability of being sampled.

%The initial estimate can be found using \Level, which has the
%lowest computational cost among the proposed methods.

%%level-based method
%One problem we left open is how to choose the level
%to be used by \Level.
%We conjecture that a more principled approach can be tailored
%based on the amount of Fisher Information contained in each level of the sample. There is
%definitely a trade-off between using obsevations closer to the root, that give
%more certainty about the true degrees, and using observations from lower levels,
%which come is larger quantities. Another issue with this method is that we are
%discarding useful information by not taking other observations into account.
%A possible future direction would be to look into how to combine all
%observations. Furthermore, if we could measure the amount of information in the
%entire sample, we will be able to derive lower bounds on estimation errors and
%use it as an actual benchmark to assess how well the three methods are performing.

%relationship with our previous work

